Towards Graph Foundation Models: Training on Knowledge Graphs Enables Transferability to General Graphs

Inspired by the success of large language models, there is a trend toward developing graph foundation models to conduct diverse downstream tasks in various domains. However, current models often require extra fine-tuning to apply their learned structural and semantic representations to new graphs, which limits their versatility. Recent breakthroughs in zero-shot inductive reasoning on knowledge graphs (KGs), offer us a new perspective on extending KG reasoning to general graph applications. In this paper, we introduce SCR, a unified graph reasoning framework designed to train on knowledge graphs and effectively generalize across a wide range of graph tasks and domains. We begin by designing the task-specific KG structures to establish a unified topology for different task formats. Then we propose semantic-conditioned message passing, a novel mechanism addressing the inherent semantic isolation in traditional KG reasoning, by jointly modeling structural and semantic invariance patterns in graph representations. To demonstrate the effectiveness, we evaluate the inductive reasoning capability of SCR using 38 diverse graph datasets, covering node-level, link-level, and graph-level tasks across multiple domains. Our results show substantial performance gains over existing foundation models and supervised baselines, highlighting the efficacy and adaptability of our approach.

==> sections/relatedwork.tex <==
\section{Related Work}

\subsection{Knowledge Graph Reasoning}

Traditional \emph{transductive} KG reasoning models, such as TransE~\citep{TransE}, DistMult~\citep{DistMult}, RotatE~\citep{RotatE}, RGCN~\citep{RGCN-ESWC18}, and CompGCN~\citep{CompGCN-ICLR20}, represent entities and relations within a knowledge graph using continuous vector embeddings~\citep{2017Survey,OurComp,OurHaLE}. 
These models, however, assume that all entities and relations in the KG are known beforehand, which limits their ability to generalize to unseen entities within the same graph or across different KGs~\citep{OurMulDE,GoogleAttH}. 
In contrast, \emph{inductive} KG reasoning approaches~\citep{NBF-NIPS21} address this limitation by enabling generalization to KGs with previously unseen entities or relations. 
Most existing inductive methods~\citep{Cycle-ICML22,InductivE-IJCNN21,IKR-JWWW23,TACT-AAAI21} employ query-conditional MPNNs to generate ``relative'' entity embeddings by extracting local structural features from a subgraph induced by the query entity. 
GraIL~\citep{GraIL-ICML19}, for example, extracts an enclosing subgraph between the query entity and each candidate entity, but this approach suffers from high computational costs. 
Other models, such as NBFNet~\citep{NBF-NIPS21} and RED-GNN~\citep{REDGNN-WWW22}, propagate query features through the $L$-hop neighborhood subgraph of the query entity. 
To improve computational efficiency, recent works have focused on optimizing algorithms, including path-pruning techniques during the GNN propagation process~\citep{Adaprop,ANet,OurGraPE}.
In the direction of building a foundation model for KG reasoning, ULTRA~\citep{ultra} utilizes four basic interaction types of the KG relational structure to perform inductive reasoning on entirely novel KGs. 
Building on ULTRA, ProLINK~\citep{OurProLINK} harnesses the power of large language models (LLMs) to enhance reasoning performance for few-shot relation types on low-resource KGs. 
Nevertheless, these inductive methods face challenges in generalizing to a wide variety of graph tasks and feature spaces, as their reasoning capabilities remain primarily confined to topological structures.

% Whether mention the text-involved KGR methods?
% text-based inductive reasoning \citep{TextKGR-BLP-WWW21, TextKGR-KEPLER-TACL21, TextKGR-StATIK-NAACL21,TextKGR-RAILD-IJCKG22}

\subsection{Graph Foundation Models}

Graph foundation models have recently gained significant attention due to their ability to handle diverse graph-structured data across a wide range of tasks.
Model fine-tuning is a straightforward way to adapt downstream tasks, but significant task differences would lead to potential negative transfer and catastrophic forgetting~\citep{rosenstein2005transfer}. Rather than fine-tuning with an adaptive task head, graph prompt learning reformulates input graph data to align with the pretext task~\citep{chen2023ultradp,tan2023virtual, gong2023prompt}.
GPF takes a prompt token as some additional features are added to the original graph. Based on that, GPF-plus~\citep{gpfplus2023} trains several independent basis vectors and utilizes attentive aggregation of these basis vectors with the assistance of several learnable linear projections.
GPPT~\citep{sun2022gppt} defines graph prompts as additional tokens that contain task tokens and structure tokens that align downstream node task and link prediction pretext. Furthermore, some works~\citep{zhu2023sglpt} use graph prompt to assist graph pooling operation (a.k.a Readout), like Gprompt~\citep{liu2023graphprompt} inserts the prompt vector to the graph pooling by element-wise multiplication.
Some studies regard graph prompt as additional graphs~\citep{ge2023enhancing,huang2023prodigy}, such as All-in-one~\citep{sun2023all} inserts the token graphs as prompt to the original graph and all links between tokens and original graphs.

Recently, several foundational models for specific graph tasks have been proposed to adapt diverse unseen data without model tuning.
ULTRA~\citep{ultra} presents a universal approach to learn transferable graph representations by conditioning on relational interactions, enabling generalization to unseen knowledge graphs. 
GraphAny~\citep{GraphAny} addresses inductive node classification by formulating inference as an analytical solution to a linear GNN architecture, while an attention module fuses predictions from multiple models, ensuring scalability. 
Models like InstructGLM~\citep{InstructGLM} and HiGPT~\citep{HiGPT} leverage large language models (LLMs), using natural language prompts to guide graph learning and handling heterogeneous graphs without downstream fine-tuning, broadening the applicability of foundation models to diverse graph tasks.
Building a general graph foundation model is not trivial; the major challenges to overcome are related to structural and feature heterogeneity.
OpenGraph~\citep{OpenGraph} proposes a zero-shot graph learning framework with a unified graph tokenizer and a scalable graph transformer, allowing the model to handle unseen graph data, aided by LLM-based data augmentation. 
AnyGraph~\citep{AnyGraph} extends this by addressing structural and feature heterogeneity through a Graph Mixture-of-Experts architecture, supporting fast adaptation and scaling efficiently. 

% However, ... 增加一句话来总结我们解决的问题。
